Realtime Rooftop Landing Site Identification and Selection in Urban City Simulation

Safe autonomous landing in urban cities is a necessity for the growing Unmanned Aircraft Systems (UAS) industry. In urgent situations, building rooftops, particularly flat rooftops, can provide local safe landing zones for small UAS. This paper investigates the real-time identification and selection of safe landing zones on rooftops based on LiDAR and camera sensor feedback. A visual high fidelity simulated city is constructed in the Unreal game engine, with particular attention paid to accurately generating rooftops and the common obstructions found thereon, e.g., ac units, water towers, air vents. AirSim, a robotic simulator plugin for Unreal, offers drone simulation and control and is capable of outputting video and LiDAR sensor data streams from the simulated Unreal world. A neural network is trained on randomized simulated cities to provide a pixel classification model. A novel algorithm is presented which finds the optimum obstacle-free landing position on nearby rooftops by fusing LiDAR and vision data.

==> Experiment.tex <==
\section{Experiment}
\subsection{Rooftop semantic segmentation}
% CLASS_NAMES = ['unknown', 'sky', 'ground', 'building_wall', 'building_rooftop','small_rooftop_entrance','skylight', 'air_vents', 'ac_unit', 'seating', 'any_ducts', 'water_tower', 'chimney', 'tarp', 'vegetation', 'power_line', 'street_light', 'door']
% Mobilenet-FCN8s
% 0.9860386 , 0.93218046, 0.9539815 , 0.97602105, 0.9137157 , 0.8331829 , 0.4312528 , 0.83798105, 0.6891968 , 0.82849056, 0.80375874, 0.89441836, 0.9196205 , 0.85471416, 0.05385061, 0.36721253, 0.72908586

We have evaluated multiple image semantic segmentation models on our proposed simulation datasets \cite{siam2018comparative}. 

\xhdr{Train dataset:} We've trained the four semantic segmentation models on a combined dataset containing 9324 images collected from 5 cities with randomly sampled rooftop objects based on statistics. All images are collected from different UAV viewpoints.

\xhdr{Test datasets:} We've evaluated the performance of different models on two datasets: a manually built city (Manual) and a randomly sampled city (Random). Each test dataset contains 1040 images collected from different UAV viewpoints. The test datasets are regenerated to ensure its independence from the training dataset.

Table~\ref{tab:per_class} shows the mean intersection over union (IOU) and per-class IOU of the four trained models.

%'sky', 'ground', 'building_wall', 'building_rooftop','small_rooftop_entrance','skylight', 'air_vents', 'ac_unit', 'seating', 'any_ducts', 'water_tower', 'chimney', 'tarp', 'vegetation'
%mean IOU:  0.7444093759570803
% Per class IOU:  [0.9939692  0.93064624 0.9627077  0.9784495  0.8209261  0.78980154
%  0.4809117  0.7790504  0.4248172  0.79821706 0.7444992  0.
%  0.900675   0.8170604 ]

% mean IOU:  0.7124080253498895

% [0.99131995 0.9153625  0.9547547  0.9729896  0.78415114 0.76714575
%  0.40560102 0.7534704  0.3743811  0.7349759  0.68347865 0.
%  0.84469205 0.7913896 ]

%segmentation size: (512, 512)
% mean IOU:  0.7286981897694724
% Per class IOU:  [0.99622333 0.935035   0.9614084  0.9757877  0.7938344  0.78675
%  0.3608551  0.7686834  0.33627015 0.7395098  0.75617194 0.
%  0.908519   0.88272643]



\begin{table*}[]
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
         & sky & ground & \makecell{building\\ wall} & \makecell{building\\ rooftop} & \makecell{small\\ rooftop\\ entrance} & \makecell{sky-\\light} & \makecell{air\\ vents} & \makecell{ac-\\unit} & \makecell{sea-\\ting} &\makecell{air-\\ducts}& \makecell{water\\ tower} & \makecell{chim-\\ney} & tarp & \makecell{vege-\\tation}  &  \makecell{Mean\\ IOU} \\
        \midrule
        \makecell{MobileNet\\ + FCN8s} & 0.99 & 0.93 & 0.96 & 0.98 & 0.82 & 0.79 & 0.48 & 0.78 & 0.42 & 0.80 & 0.74 & N/A & 0.90 & 0.81 & 0.74 \\
        \midrule
        \makecell{ShuffleNet\\ + FCN8s} &&&&&&&&&&&& &  & 0.71 \\
        \midrule
        \makecell{MobileNet\\ + UNet} &&&&&&&&&&&&&& 0.\\
        \midrule
        \makecell{ShuffleNet\\ + UNet} &&&&&&&&&&&&&& 0.\\
        \bottomrule
    \end{tabular}
    \caption{Results of different image semantic segmentation networks on our urban rooftop dataset}
    \label{tab:per_class}
\end{table*}

\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
         &  \multicolumn{2}{c|}{RTX 2080} & \multicolumn{2}{c|}{TX2 (TensorFlow)} & \multicolumn{2}{c}{TX2 (TensorRT)} \\
         \cline{2-7}
         & mIOU &  time(ms) & mIOU & time(ms) & mIOU & time(ms) \\
        \hline
        \makecell{MobileNet\\ + FCN8s} & 0.76 & 8.17 & 0.76 & 147.93 &  & 89 \\ %164
        \makecell{ShuffleNet\\ + FCN8s} & 0.74 & 9.94 & 0.74 & 146.70 & & 71 \\ %184
        \makecell{MobileNet\\ + UNet} & 0.74 & 17.09 & & 277.62 & & \\
        \makecell{ShuffleNet\\ + UNet} & 0.74 & 17.09 & & 277.62 & & \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
% number of nodes:
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
        model & origin & remove train & strip switch/identity & trt optimized \\
        \makecell{MobileNet\\ + FCN8s} & 1003 & 752 & 425 & 292 \\
        \makecell{ShuffleNet\\ + FCN8s} & 2623 & 2071 & 1524 & 985 \\
        \makecell{MobileNet\\ + UNet} & 1258 & 942 & 531 & 358 \\ 
        \makecell{ShuffleNet\\ + UNet} & 2951 & 2319 & 1668 & 1070
    \end{tabular}
    \caption{Number of operation nodes}
    \label{tab:nodes}
\end{table}

It can be seen that the FCN8s meta-architecture with MobileNet backbone achieves the highest mean IOU on our testing dataset. 
\begin{figure}[hp]
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/seg_example.png}
    \caption{Semantic segmentation on rooftop image in our dataset.}
    \label{fig:seg_example}
\end{figure}


% # MobileNet FCN8s on Validation dataset
% Model: FCN8sMobileNet 
% Time: 7.832049 
% Mean_iou: 0.764982 
% per class iou: [0.9860386  0.93218046 0.9539815  0.97602105 0.9137157  0.8331829
%  0.4312528  0.83798105 0.6891968  0.82849056 0.8037586  0.89441836
%  0.9196205  0.85471416 0.05385061 0.36721253 0.72908586]

% # MobileNet FCN8s on CV_Manual
% Model: FCN8sMobileNet 
% Time: 8.17
% Mean_iou: 0.596185
% per class iou: [0.99179333 0.90360403 0.9521174  0.9702189  0.32610297 0.5433829
%  0.39259246 0.5730579  0.5097603  0.40318882 0.7335166  0.4484017
%  0.9407307  0.8079401  0.00115699 0.1541514  0.48342228]

% # MobileNet FCN8s on CV_Random_Histogram
% Model: FCN8sMobileNet 
% Time: 9.52
% Mean_iou: 0.626081
% per class iou: [0.9934262  0.9044864  0.9521618  0.9743431  0.7285827  0.79020447
%  0.38681448 0.74757016 0.3317044  0.7380395  0.6479621  0.
%  0.8933653  0.7890229  0.00248895 0.16101108 0.6021979 ]
    

% # ShuffleNet FCN8s on Validation dataset
% Model: FCN8sShuffleNet 
% Time: 9.939567 
% Mean_iou: 0.740697 
% per class iou: [0.9819374  0.92100424 0.9454226  0.97071713 0.8919036  0.8143741
%  0.4096751  0.8093346  0.65112555 0.7875616  0.7752348  0.8792261
%  0.90480435 0.8371956  0.03003817 0.2609902  0.72130483]

% # ShuffleNet FCN8s on Manual dataset
% Model: FCN8sShuffleNet 
% Time: 10.504624 
% Mean_iou: 0.567525 
% per class iou: [0.9892236  0.8827247  0.94396925 0.9647412  0.3149243  0.5055409
%  0.3447977  0.527146   0.45395857 0.33124483 0.71106094 0.48916465
%  0.92860883 0.79295146 0.         0.07508529 0.39277738]

% # ShuffleNet FCN8s on CV_Random_Histogram dataset
% Model: FCN8sShuffleNet 
% Time: 9.426008 
% Mean_iou: 0.593292 
% per class iou: [0.99086666 0.8868926  0.9431177  0.9681425  0.6957779  0.75316083
%  0.3502395  0.6926213  0.27422947 0.6553712  0.60759914 0.
%  0.8660416  0.7693265  0.0026532  0.08100874 0.5489082 ]
    
% # UNetMobileNet on validation dataset
% Model: UNetMobileNet 
% Time: 16.910503 
% Mean_iou: 0.739837 
% per class iou: [0.9931862  0.9114253  0.94876796 0.9679644  0.88279146 0.84102774
%  0.3548003  0.8069735  0.6990636  0.8250702  0.79234517 0.86773676
%  0.92135257 0.8975703  0.         0.25308433 0.61407715]

% # UNetMobileNet on CV_Manual dataset
% Model: UNetMobileNet 
% Time: 17.204221 
% Mean_iou: 0.585809 
% per class iou: [0.9954737  0.9062105  0.9517449  0.9709318  0.2903634  0.52976316
%  0.35386142 0.57233644 0.47491732 0.30348706 0.7440301  0.5686643
%  0.942558   0.8777512  0.         0.09490521 0.38176093]
    
% # UNetMobileNet on CV_Random_Histogram dataset
% Model: UNetMobileNet 
% Time: 17.085816 
% Mean_iou: 0.601225 
% per class iou: [0.9960176  0.8513305  0.9539146  0.9607809  0.6875438  0.8046355
%  0.36736372 0.7270763  0.30880427 0.7387913  0.73967934 0.
%  0.5588881  0.86241406 0.         0.09831192 0.56527215]
